Auto-Vocabulary Semantic Segmentation

Open-Vocabulary Segmentation (OVS) methods are capable of performing semantic segmentation without relying on a fixed vocabulary, and in some cases, without training or fine-tuning. However, OVS methods typically require a human in the loop to specify the vocabulary based on the task or dataset at hand. In this paper, we introduce Auto-Vocabulary Semantic Segmentation (AVS), advancing open-ended image understanding by eliminating the necessity to predefine object categories for segmentation. Our approach, AutoSeg, presents a framework that autonomously identifies relevant class names using semantically enhanced BLIP embeddings and segments them afterwards. Given that open-ended object category predictions cannot be directly compared with a fixed ground truth, we develop a Large Language Model-based Auto-Vocabulary Evaluator (LAVE) to efficiently evaluate the automatically generated classes and their corresponding segments. With AVS, our method sets new benchmarks on datasets PASCAL VOC, Context, ADE20K, and Cityscapes, while showing competitive performance to OVS methods that require specified class names.

==> Sections/1_introduction_old.tex <==
\section{Introduction}
Semantic segmentation is a computer vision task that involves grouping pixels into coherent regions based on their semantic categories. While notable advancements have been made, existing semantic segmentation models primarily rely on labeled datasets with predefined categories, limiting their ability to handle unknown classes. In contrast, humans possess an open-ended understanding of scenes, recognizing thousands of distinct categories. Recent studies have focused on the development of segmentation models to meet similar capabilities~\cite{weak-sup1, self-sup1}, with models that leverage Vision-Language Models (VLMs) as an emerging category~\cite{lseg, openseg, maskclip, ovseg, catseg, fcclip, opsnet,san, simseg}. Such VLMs learn rich multi-modal features from large numbers of image-text pairs.
\begin{figure}[t!]
  \centering
  \includegraphics[width=\linewidth]{Figures/teaser.pdf}\\
  \caption{\textbf{\ours Exemplary Results.} While established segmentation datasets have a fixed set of annotation categories, our method is able to identify and segment object categories beyond the fixed-set ground truth, such as \textit{cub}, \textit{dachshund} or \textit{pagoda}.
  Images are from the PASCAL VOC~\cite{VOC} and ADE20K~\cite{ADE20k} datasets.}
  \label{fig:teaser}
\end{figure}

%
\begin{figure*}[ht!]
  \centering
  \includegraphics[width=\linewidth]{Figures/different_segmentation_tasks.pdf}\\
  \caption{\textbf{Different Semantic Segmentation Tasks in Comparison.} In traditional Semantic Segmentation, an image is segmented into fixed, predefined dataset classes used during annotation. In Open-Vocabulary Segmentation, the user specifies which object categories (from the open vocabulary) need to be segmented. In Auto-Vocabulary Segmentation, relevant object categories are generated from the image automatically, enabling a true open-ended understanding of scenes without a human in the loop.}
  \label{fig:diff_seg_tasks}
\end{figure*}
%

%
Given the scale, training VLMs comes at a extremely high computational cost. Because of this, it is common to build upon pre-trained VLMs such as CLIP~\cite{clip} or BLIP~\cite{blip}. However, applying these VLMs on per-pixel tasks is non-trivial, as they are trained on full images and lack the ability to directly reason over local regions in the image. Previous attempts have employed a two-stage approach where masked regions are fed to the VLMs to produce CLIP embeddings, which are subsequently correlated with text encodings of text prompts to perform classification~\cite{zsseg, ovseg, maskclip}. Other works directly align per-pixel embeddings with text embeddings retrieved from CLIP~\cite{lseg} based on text prompts provided by the user at test time. While training these models, the text prompts usually correspond to the ground truth class names of the dataset in question. In this paper, we take the capabilities of VLMs one step further and tackle a more challenging task in which the relevant class names are automatically generated. We enable \textit{Auto-Vocabulary Semantic Segmentation (AVS)}, in which the goal is to produce accurate object segmentation and their pixel-level classifications for \textbf{any} class without the need for textual input from the user, predefined class names, additional data, training or fine-tuning.

To tackle this task, we introduce the \ours framework. Our framework can adapt to any Open-Vocabulary Segmentation (OVS) backbone. We propose \textsc{BLIP-Cluster-Caption (BCC)} to generate relevant class names, consisting of four simple steps: 1) obtain local BLIP embeddings at different image scales; 2) cluster local BLIP embeddings to identify and separate meaningful semantic areas in the image; 3) caption each clustered embedding and extract nouns from the caption; and 4) pass the resulting nouns to a pre-trained segmentation backbone as class names, thereby essentially creating a self-guided network.

Experimental evaluations on PASCAL VOC~\cite{VOC} and Context~\cite{context}, ADE20K~\cite{ADE20k} and Cityscapes~\cite{cityscapes} showcase the effectiveness of \ours, achieving state-of-the-art results on AVS and results competitive to OVS methods which are - unlike \ours - limited by the need for pre-specified class names. It is capable of predicting crisp segmentation masks without having any information a priori about which objects to segment (see Fig.~\ref{fig:teaser}). For effective evaluation on public datasets, we furthermore propose a Large Language Model-based Auto-Vocabulary Evaluator (\textsc{LAVE}), tasked with mapping auto-vocabulary predictions to fixed ground truth class names in the dataset. All code will be publicly released to ensure reproducibility and to facilitate further research into AVS.

In summary, our contributions are as follows: 
\textbf{1)} we introduce \ours, a novel framework to automatically determine and segment relevant classes in an image; 
\textbf{2)} we propose \textsc{BLIP-Cluster-Caption}, a novel image captioning method capable of generating local and semantically meaningful descriptions from the image obtained from enhanced BLIP embeddings; and 
\textbf{3)} we propose \textsc{LAVE}, a novel evaluation method for auto-vocabulary semantic segmentation which utilizes an LLM. Through qualitative and quantitative analyses, we demonstrate the effectiveness of our framework for Auto-Vocabulary Semantic Segmentation on multiple public datasets.

==> Sections/1_introduction_old2.tex <==

\section{Introduction}
Despite advancements in semantic segmentation, existing models rely heavily on labeled datasets with predefined categories, limiting their ability to handle unknown classes. In contrast, humans possess an open-ended understanding of scenes, recognizing thousands of distinct categories. Recent work has focused on leveraging Vision-Language Models (VLMs)~\cite{lseg, openseg, maskclip, ovseg, catseg, fcclip, opsnet, san, simseg} to capture a more open-ended understanding of scenes by learning multi-modal features from large-scale image-text pairs. 
%Semantic segmentation is a computer vision task that involves grouping pixels into coherent regions based on their semantic categories. While notable advancements have been made, existing semantic segmentation models primarily rely on labeled datasets with predefined categories, limiting their ability to handle unknown classes. In contrast, humans possess an open-ended understanding of scenes, recognizing thousands of distinct categories. Recent studies have focused on the development of segmentation models to meet similar capabilities~\cite{weak-sup1, self-sup1}, with models that leverage Vision-Language Models (VLMs) as an emerging category~\cite{lseg, openseg, maskclip, ovseg, catseg, fcclip, opsnet,san, simseg}. Such VLMs learn rich multi-modal features from large numbers of image-text pairs.
%
\begin{figure*}[ht!]
  \centering
  \includegraphics[width=\linewidth]{Figures/different_segmentation_tasks.pdf}\\
  \caption{\textbf{Semantic Segmentation Tasks in Comparison.} In traditional Semantic Segmentation, an image is segmented into fixed, predefined set of classes (fixed vocabulary). In Open-Vocabulary Segmentation, the user specifies which object categories (from the open vocabulary) should be segmented: 1) either via a human-provided prompt at runtime, or 2) the OV-method is trained to output the vocabulary of a human-annotated target dataset. In contrast, for Auto-Vocabulary Segmentation, relevant object categories are generated from the image automatically, enabling a true open-ended understanding of scenes without a human in the loop.}
  \label{fig:diff_seg_tasks}
\end{figure*}
%
%Given the scale, training VLMs comes at a extremely high computational cost. Because of this, it is common to build upon pre-trained VLMs such as CLIP~\cite{clip} or BLIP~\cite{blip}. However, applying these VLMs on per-pixel tasks is non-trivial, as they are trained on full images and lack the ability to directly reason over local regions in the image. 
Due to the high computational cost of training VLMs, most approaches build on pre-trained models like CLIP\cite{clip} or BLIP~\cite{blip}. However, applying these VLMs to per-pixel tasks is challenging, as they are trained on full images and lack local reasoning capabilities.
Previous attempts have employed two-stage approaches which correlate CLIP embeddings from masked regions with text prompt encodings to perform classification~\cite{zsseg, ovseg, maskclip}. Other works directly align per-pixel embeddings with text embeddings retrieved from CLIP~\cite{lseg} based on text prompts provided by the user at test time. While training these models, the text prompts typically correspond to the ground truth class names of the dataset in question. In this paper, we take the capabilities of VLMs one step further and tackle a more challenging task in which the vocabulary is unknown a priori and target class names are automatically generated. We enable \textit{Auto-Vocabulary Semantic Segmentation (AVS)}, in which the goal is to produce accurate object segmentation and their pixel-level classifications for \textbf{any} class without the need for textual input from the user, predefined class names, additional data, training or fine-tuning. Fig.~\ref{fig:diff_seg_tasks} shows the different settings. Our method's independence from human supervision, ability to generalize to any target class in zero-shot manner, as well as its ability to scale to any vocabulary size makes it ideal for applications with open-ended characteristics, such as robot navigation or autonomous driving where new object categories are continually encountered.

To address this task, we present the \ours framework, which begins by identifying target categories and predicts masks for them. We propose \blip to generate a scene-specific target vocabulary for each image, consisting of three steps: 1) obtain vision-language embeddings at different image scales with BLIP; 2) separate and enhance vision-language embedding tokens into semantic token clusters over multiple generation cycles; and 3) decode sentences from each semantic token cluster and extract nouns. To the best of our knowledge, we are the first to use the text decoder in this manner, enabling object-level captioning for which it was never specifically trained. The final segmentation of all open-ended target classes is performed with a pre-trained segmentation backbone.

Comparing \ours's quantitative performance on public benchmarks presents a unique challenge. Open-ended class predictions cannot be directly compared to a fixed ground truth (e.g., \textit{pagoda} versus \textit{building} in Fig. \ref{fig:teaser}). This challenge is further complicated when predicted regions lack corresponding annotations (e.g., a \textit{bed} prediction labeled as \textit{background} in Fig. \ref{fig:teaser}). To bridge the gap between auto-generated and fixed vocabularies, we introduce the Large Language Model-based Auto-Vocabulary Evaluator (\textsc{LAVE}). \textsc{LAVE} is designed to map auto-vocabulary predictions to the fixed ground truth vocabulary based on semantic similarity. To promote reproducibility and support further research in AVS, we will publicly release all code.

Experimental evaluations, enabled by \textsc{LAVE}, on PASCAL VOC~\cite{VOC} and Context~\cite{context}, ADE20K~\cite{ADE20k} and Cityscapes~\cite{cityscapes} showcase the effectiveness of \ours in open-ended recognition, achieving state-of-the-art results on AVS and results competitive to OVS methods which rely - unlike \ours - on a pre-specified vocabulary. Without prior knowledge of target classes, our method still effectively segments relevant objects (see Fig.~\ref{fig:teaser} and Fig.~\ref{fig:qualitative}). 

In summary, our contributions are as follows: 
\textbf{1)} we introduce \ours, a novel framework to automatically determine and segment open-ended classes in an image; \textbf{2)} we propose \blip, a novel method for generating image-specific target vocabularies, leveraging text decoding from enhanced BLIP embeddings; and \textbf{3)} we propose \textsc{LAVE}, a novel evaluation approach for auto-vocabulary semantic segmentation which utilizes an LLM. Through qualitative and quantitative analyses, we demonstrate the effectiveness of our framework for Auto-Vocabulary Semantic Segmentation on multiple public datasets.

==> Tables/captioning_models.tex <==
\begin{table}[tb]
\caption{\textbf{Experiments with Alternative Class Generation Baselines (mIoU).} Experiments with alternative methods to generate classes showcase that \ours is favorable for AVS across all three datasets, with larger performance gaps on VOC and Cityscapes with a smaller vocabulary size.}
\centering
\footnotesize
\setlength{\tabcolsep}{8pt} 
\renewcommand{\arraystretch}{1.2}
\newcommand{\csp}{\hskip 2em}
\begin{tabular}{l ccc}
\toprule
\textbf{Approach} & \textbf{VOC}~\cite{VOC} & \textbf{PC}~\cite{context} & \textbf{CS}~\cite{cityscapes} \\
\midrule
\textsc{SAM} + \textsc{BLIP} + \textsc{X-Decoder} & \rd 41.1 & \rd 11.3 & \rd 27.4 \\
\textsc{LLAVA} + \textsc{X-Decoder}               & \nd 56.7 & \nd 11.4 & \nd 23.4 \\
\ours (Ours)                                      & \fs 87.1 & \fs 11.7 & \fs 29.5 \\
\bottomrule
\end{tabular}%}
\label{tab:captioning}
\vspace{-10pt}
\end{table}
